A TTL-based Approach for Content Placement in Edge Networks

Edge networks are promising to provide better services to users by provisioning computing and storage resources at the edge of networks. However, due to the uncertainty and diversity of user interests, content popularity, distributed network structure, cache sizes, it is challenging to decide where to place the content, and how long it should be cached. In this paper, we study the utility optimization of content placement at edge networks through timer-based (TTL) policies. We propose provably optimal distributed algorithms that operate at each network cache to maximize the overall network utility. Our TTL-based optimization model provides theoretical answers to how long each content must be cached, and where it should be placed in the edge network. Extensive evaluations show that our algorithm significantly outperforms path replication with conventional caching algorithms over some network topologies.

==> 05-discussion-mcdp.tex <==





In this section, we provide some discussions on our utility maximization framework under MCDP for edge networks.  %We first consider the case of general network topology with overlapping paths.
We first consider a direct application to content distributions in CDNs, ICNs etc., % in Section~\ref{sec:app}, 
 and then discuss the costs incurred for content placement in edge networks.% in Section~\ref{sec:cost}.

%\subsection{Application}\label{sec:app}
\input{05-app-cdn}
%
%\vspace{-0.05in}
%\subsection{Minimizing Cost}\label{sec:cost}
\input{05-min-cost}
